On Statistical Bias In Active Learning: How and When To Fix It

Active learning is a powerful tool when labelling data is expensive, but it introduces a bias because the training data no longer follows the population distribution. We formalize this bias and investigate the situations in which it can be harmful and sometimes even helpful. We further introduce novel corrective weights to remove bias when doing so is beneficial. Through this, our work not only provides a useful mechanism that can improve the active learning approach, but also an explanation of the empirical successes of various existing approaches which ignore this bias. In particular, we show that this bias can be actively helpful when training overparameterized models -- like neural networks -- with relatively little data.

==> active_evaluation.tex <==
\section{Active Evaluation}
However, even if bias can be useful for model training for certain kinds of model, what if we are trying to estimate the population risk of a trained model?
Ordinarily, active learning ignores testing.
However, the labels we use for testing are just as expensive as the labels we use for training.
It therefore makes sense to consider sample-efficient evaluation.
In Figure \ref{fig:model_evaluation} we show how a \seb{fill in with exp}

==> note_on_inequality.tex <==

Consider the expression:
\begin{align}
    &\sum_{m=1}^{M} \frac{(N-M)^2}{(N-m)^2} < \sum_{m=1}^{M}\frac{(N-m+1)^2}{N^2}.
\end{align}

The left hand side is an increasing function in $m$. 
Therefore, we can put an upper bound on the left hand side with an integral:
\begin{align}
    \sum_{m=1}^{M} \frac{(N-M)^2}{(N-m)^2}
     &\leq \int_{m=2}^{M+1} \frac{(N-M)^2}{(N-m)^2}\\
     & \leq \left[-\frac{(M-N)^2}{m-N}\right]^{M+1}_{2}\\
     & \leq (M-N)^2\left(\frac{1}{2-N} - \frac{1}{M+1-N}\right)\\
     & \leq (M-N)^2\frac{M-1}{(N-2)(N-M-1)}
 \end{align}
 The right hand side can be found exactly:
 \begin{align}
    \sum_{m=1}^{M}&\frac{(N-m+1)^2}{N^2} \\
   &= \frac{1}{N^2}\sum_{m=1}^{M} m^2 - m(N+1) + (N+1)^2\\
   &= \frac{1}{N^2}\left(\frac{M(M+1)(2M+1)}{6} - M(N+1)(M+1) + M(N+1)^2\right).
 \end{align}
 The difference can be written:
 \begin{align}
     \frac{2M^4N - 4M^4 -2M^3N^2 + 16 M^3N +M^3 -27M^2N^2 + 4 M^2 + 24MN^3 -9MN -2M -6N^4}{6N^2(N-2)(M-N+1)}
 \end{align}
